From PowerPoint UI Sketches to Web-Based Applications: Pattern-Driven Code Generation for GIS Dashboard Development Using Knowledge-Augmented LLMs, Context-Aware Visual Prompting, and the React Framework

Developing web-based GIS applications, commonly known as CyberGIS dashboards, for querying and visualizing GIS data in environmental research often demands repetitive and resource-intensive efforts. While Generative AI offers automation potential for code generation, it struggles with complex scientific applications due to challenges in integrating domain knowledge, software engineering principles, and UI design best practices. This paper introduces a knowledge-augmented code generation framework that retrieves software engineering best practices, domain expertise, and advanced technology stacks from a specialized knowledge base to enhance Generative Pre-trained Transformers (GPT) for front-end development. The framework automates the creation of GIS-based web applications (e.g., dashboards, interfaces) from user-defined UI wireframes sketched in tools like PowerPoint or Adobe Illustrator. A novel Context-Aware Visual Prompting method, implemented in Python, extracts layouts and interface features from these wireframes to guide code generation. Our approach leverages Large Language Models (LLMs) to generate front-end code by integrating structured reasoning, software engineering principles, and domain knowledge, drawing inspiration from Chain-of-Thought (CoT) prompting and Retrieval-Augmented Generation (RAG). A case study demonstrates the framework's capability to generate a modular, maintainable web platform hosting multiple dashboards for visualizing environmental and energy data (e.g., time-series, shapefiles, rasters) from user-sketched wireframes. By employing a knowledge-driven approach, the framework produces scalable, industry-standard front-end code using design patterns such as Model-View-ViewModel (MVVM) and frameworks like React. This significantly reduces manual effort in design and coding, pioneering an automated and efficient method for developing smart city software.

==> Backup/backup.tex <==



%aims to lower the technical barriers and cost to the development of advanced scientific software to facilitate urban and environmental management within smart city initiatives.


 

%This research introduces a system-based methodology to automate the development of sophisticated web-based GIS applications to support urban and environmental management within smart city initiatives. By employing ontology-driven prompts and large language models (LLMs), our approach leverages the AI's capabilities in generation, reasoning, and learning to create a primitive autonomous agent that assists academic researchers and prospective developers by lowering both the technical barriers and costs associated with developing cyberinfrastructure and scientific software tools. Technically, we have developed a prototyping framework that creates a Knowledge Graph (KG) to digitally represent software engineering practices, popular application stacks, package management tools, and domain-specific knowledge of data and simulations. The KG is later used to generate, tune, and enhance engineered prompts through iterative procedures, providing precise instructions for the ChatGPT 4.0 API, DALL-E API, and LangChain to automate the development of geo-visual dashboards using web frameworks and technologies favored by the industry. We demonstrate the effectiveness and feasibility of our framework with a case study of an AI-generated visual dashboard of atmospheric and dispersion data from real-time sensors, machine learning analytics, and environmental simulations using the React framework and Python Tornado server. This study investigates the potential of LLMs to function as full-stack web developers and GIS analysts. By leveraging scientific KGs, the LLMs are guided to comprehend advanced software design and architecture patterns, such as MVC and MVVM, as well as complex scientific data, illuminating the autonomous development of robust, generalized, and scalable geospatial web applications that perform efficiently on both the server and client sides.


%This pipeline leverages urban
%science domain ontologies to transform scientific concepts (datasets, simulation models, metrics, AI algorithms) into software components using robust design patterns. Utilizing LLMs for natural language understanding, reasoning, and coding, it automatically implements these components in popular programming languages. Our AI-powered urban digital twins offer advanced capabilities: real-time IoT data visualization, multi-objective decision optimization, and predictive analytics for urban dynamics. We validate our pipeline with three smart city case studies focusing on freight transportation management, urban climate modeling, and building energy optimization. Implemented using the GPT-4 API in a Python environment, our pipeline synergizes with knowledge graphs created using prevalent ontology languages. The results are compelling: for each case study, the pipeline efficiently generated operational digital twins using an MVC-based Python framework. This marks a significant reduction in manual software design and coding efforts. Our research presents a pioneering path towards next-generation AI-powered urban digital twins that are self-generating, self-organizing, and self-executing, demonstrating the transformative potential of LLMs in urban technology development.



%The study develops 
%The study develops formal models, both information and functional, and establishes the methodological foundations for integrating ontology-driven prompts with ChatGPT's meta-learning capabilities. The resulting productive triad comprises the methodological foundations, advanced information technology, and the OntoChatGPT system, which collectively enhance the effectiveness and performance of chatbot systems. The implementation of this technology is demonstrated using the Ukrainian language within the domain of rehabilitation. By applying the proposed methodology, the OntoChatGPT system effectively extracts entities from contexts, classifies them, and generates relevant responses. The study highlights the versatility of the methodology, emphasizing its applicability not only to ChatGPT but also to other chatbot systems based on LLMs, such as Google's Bard utilizing the PaLM 2 LLM. The underlying principles of meta-learning, structured prompts, and ontology-driven information retrieval form the core of the proposed methodology, enabling their adaptation and utilization in various LLM-based systems. This versatile approach opens up new possibilities for NLP and dialogue systems, empowering developers to enhance the performance and functionality of chatbot systems across different domains and languages.


%Large Language Models (LLMs) have revolutionized fields ranging from creative writing to code generation with their deep understanding of human language. In this paper, we harness the LLMs' capabilities to automate the full-stack web application development of GIS-based scientific visual dashboard to support environmental management and
%smart city research. 

Developing web-based dashboards for advanced querying, visualization, and interaction with GIS data in environmental research often requires repeated, costly software development. While generative AI (GenAI) code generation shows promise, it faces challenges in handling complex scientific software that demands domain expertise, advanced software engineering practices, and intricate user workflows, due to the token limits and attention capabilities of current large language models (LLMs). To address these challenges, this paper presents a knowledge-driven framework that leverages knowledge representations in software engineering, scientific data, simulations, and software stacks to instruct and fine-tune Generative Pre-trained Transformers (GPT). This enables an autonomous software development workflow for generating code for sophisticated web applications, such as CyberGIS dashboards and visual analytics interfaces, from user-defined GUI wireframes sketched in PowerPoint or other graphical design tools (e.g., Adobe Illustrator). The prototyping workflow was implemented in Python using cutting-edge Generative AI and software engineering technologies, including the ChatGPT API and a local Ollama instance, within a RAG (Retrieval-Augmented Generation) paradigm that leverages Knowledge Graphs (KG) and vector databases. We demonstrate the feasibility and effectiveness of our framework through a case study that autonomously created a web-based platform that entails multiple visualization dashboards of environmental and energy data (e.g., time-series and spatial) based on user-defined visual prompts. The platform was built following industry-standard software engineering practices, such as Single-Page Application (SPA) and Model-View-ViewModel (MVVM) architecture patterns, that are modular, generalizable, reusable, and maintainable. Our work demonstrates the potential to reduce manual software design, coding, and maintenance efforts by guiding GenAI with software engineering knowledge, pioneering an autonomous and scalable approach for generating complex web applications to facilitate urban and environmental management within the smart city initiatives

In the past decades, scientific web applications (Web Apps), such as CyberGIS systems, visual analytical dashboards, digital twin platforms, and online decision support systems, have become indispensable tools for enabling both the scientific community and the public to discover, query, visualize, and download vast amounts of urban and environmental datasets in smart city research \citep{ferre2022adoption, dembski2020urban}. Aligned with the NSF's cyberinfrastructure (CI) initiative, academia and governmental science agencies have increasingly developed and adopted web applications as part of interdisciplinary informatics projects to serve as effective, user-friendly tools for cyber-delivery \citep{yu2021coevolution}. With advancements in internet and communication technologies, computing hardware, and artificial intelligence, these tools are transforming urban and environmental research by enabling data- and simulation-driven insights for decision support and optimization\citep{kadupitige2022enhancing}, fostering collaborative research through data and simulation sharing and integration \citep{parashar2019virtual}, and enhancing education and public engagement for citizen science and voluntary data collection \citep{skarlatidou2019volunteers} across various smart city disciplines. Notable application disciplines include water resources management \citep{souffront2018cyberinfrastructure, xu2022overview}, hazard mitigation \citep{mandal2024prime, xu2020web, garg2018cloud}, intelligent transportation systems \citep{xu2023smart, xu2022interactive, ghosh2017intelligent}, connected and automated vehicles\citep{xu2023mobile, kampmann2019dynamic}, built-environment management \citep{jia2019adopting, kim2022design}, and urban planning and design \citep{alatalo2017two}. Numerous interdisciplinary studies have demonstrated the transformative and unique capabilities of these scientific web applications in advancing environmental and urban research, as well as smart city management. Their continuous evolution is driven by the integration of emerging technologies such as artificial intelligence, the Internet of Things (IoT), edge computing, and cyber-physical systems. 

Despite the significant advancements in developing scientific web applications, creating customized software tools, such as cyberGIS and digital twin platforms for integrating and visualizing diverse types of environmental or urban data, such as hydrological data, traffic flow data, meteorological data, or simulation outputs, remains a highly demanding and resource-intensive task \citep{shanjun2024design, siddiqui2024digital, lei2023challenges}. These efforts require not only substantial expertise in software engineering and data engineering, but also considerable time spent on both client-side and server-side development, as well as database management, real-time data analytics, machine learning integration, and simulations \citep{ikegwu2022big}. As a result, urban and environmental researchers are often diverted from their core scientific and analytical work to learn complex web programming languages, frameworks, visualization libraries, UI/UX design principles, and database technologies \citep{li2022bibliometric}. Although modern software engineering practices, such as design patterns and architecture patterns, aim to streamline development and ensure maintainability, their effective use still requires specialized knowledge in software engineering \citep{fayad2015software}. Researchers, who may have programming expertise in data analytics but often lack formal software development experience, face challenges in applying these practices effectively \citep{kim2017data}. Even with the involvement of skilled software engineers, designing, developing, deploying, and maintaining large-scale scientific web applications remains a labor-intensive process, requiring repetitive and costly efforts \citep{shah2024optimizing, mcbreen2002software}. This hinders the scalability, flexibility, and adaptability of platforms like cyberGIS or digital twins, limiting their ability to incorporate new data types, extend to larger geographic regions, or enhance predictive analytics and decision support capabilities \citep{liu2015cybergis, lei2023challenges}. Given these challenges, there is a growing need to leverage emerging Generative AI (GenAI) technologies to automate various aspects of web application development to support environmental and urban research. Many contemporary studies have explored the potential and feasibility of training generative AI models, particularly Large Language Models (LLMs) and specialized variants like Generative Pretrained Transformers (GPT), to act as software developers by generating code for automating simple data analytics and software development tasks \citep{liang2024can, liukko2024chatgpt}. However, developing complex scientific web apps, such as cyberGIS platforms for querying and visualizing domain-specific environmental data across multiple sites, remains challenging. These challenges arise from the inefficiency and lack of systematic and graphical prompting methods, as well as the limitations in domain and software engineering knowledge, and attention mechanisms within current LLMs that are pre-trained using generalized text data.

==> Backup/backup_lit.tex <==

\subsection{The Raise of Transformer-based Language Models}

\subsection{Review of LLM in Software Engineering}
\citep{hou2023large} provides a comprehensive review of how large language models (LLMs) are being applied in software engineering (SE). The paper categorizes LLMs into different architectures such as encoder-only, encoder-decoder, and decoder-only models and analyzes their applications across various SE tasks like requirements engineering, code generation, bug fixing, program repair, and vulnerability detection. One of the key contributions is identifying the growing trend of using decoder-only models (e.g., GPT series) for automating code generation and completion tasks, showcasing their capability in reducing manual coding effort. However, challenges remain, including handling domain-specific knowledge, improving dataset quality, and managing the complexity of SE tasks that require more than simple text generation. The paper highlights the need for better preprocessing of data, fine-tuning of models for specific SE tasks, and the importance of using diverse datasets, particularly from industrial contexts, which are currently underrepresented in research. Future work proposes addressing these challenges through more focused studies on dataset variety, improving the robustness of LLMs in handling complex SE tasks, and refining evaluation metrics for assessing LLM performance in real-world SE environments. This paper significantly contributes to the field by providing a roadmap for future research in automating software development using LLMs, emphasizing the potential of these models to assist but not yet fully replace human developers in complex SE processes. 

\citet{fan2023large} provides an in-depth overview of how large language models (LLMs) like GPT, BERT, and Codex are being integrated into various software engineering tasks such as code generation, program repair, and automated testing. The paper identifies significant contributions to the automation of software development through generative AI, particularly in areas like automated code completion, bug detection, and software refactoring. It highlights how LLMs have revolutionized these tasks by reducing the manual effort required, improving coding efficiency, and enhancing developer productivity. However, the paper also notes several challenges, such as LLMs’ tendency to produce hallucinations (i.e., incorrect but plausible outputs), difficulties with domain-specific tasks, and the need for fine-tuning models to better suit specific software engineering contexts. It also mentions the problem of non-deterministic outputs from LLMs, which complicates scientific evaluation. Furthermore, the oracle problem persists in evaluating the correctness of generated solutions. The authors propose several areas for future work, including improving prompt engineering, hybridizing LLMs with traditional software engineering methods, and further research into how LLMs can be applied to underexplored areas like requirements engineering and software design. The integration of automated testing techniques with LLM outputs is also suggested as a way to mitigate hallucination and improve overall reliability.

\subsection{Evaluating LLM for Software Development}

\citet{liang2024can} explores the potential of GPT-4, a large language model (LLM), to replicate empirical software engineering research by identifying key assumptions and generating code for analysis pipelines. Through a user study involving 14 participants and seven empirical software engineering papers, the study found that GPT-4 could successfully surface correct assumptions, but it struggled with common knowledge and relevance, often lacking domain-specific expertise in software engineering. Although GPT-4 generated high-level analysis plans that accurately outlined research methodologies, the code it produced frequently contained errors such as incorrect data sources, missing steps, and implementation-level mistakes. Only 30\% of the generated code was executable without modifications. Despite these limitations, the study highlights GPT-4’s ability to provide a useful scaffold for automating parts of the software engineering process, particularly in replicating studies and creating analysis pipelines. GPT-4 can assist with brainstorming assumptions and structuring analysis code, potentially accelerating software development. However, due to its limitations, human oversight remains crucial for correcting errors and ensuring the accuracy and reliability of the generated code.
\citep{sandberg2024evaluating} investigates GPT-4’s ability to automate the development of full-stack web applications, examining both front-end and back-end generation. The study evaluates three web applications of varying complexity and analyzes key metrics such as prompt efficiency, debugging effort, and code quality. The findings highlight that GPT-4 can successfully generate functional applications, offering the advantage of speeding up the development process, especially for simpler projects. However, as application complexity increases, the tool struggles with debugging and handling intricate integrations, requiring significant human intervention. While GPT-4 can effectively generate foundational code, its limitations in dealing with complex logic, debugging, and quality assurance present notable challenges. This study underscores GPT-4’s role as a valuable assistant in automating parts of software development but not as a fully autonomous solution for complex systems, where human expertise remains essential.

\subsection{Existing GenAI Applications for Software Engineering}


\citep{phan2024hyperagent} introduces a novel multi-agent system designed to address a wide variety of software engineering (SE) tasks. HyperAgent consists of specialized agents (Planner, Navigator, Code Editor, and Executor) that mimic typical developer workflows, managing tasks from planning to execution. Through extensive evaluations on diverse benchmarks (SWE-Bench, RepoExec, and Defects4J), the system demonstrated superior performance in tasks such as GitHub issue resolution, repository-level code generation, and fault localization. HyperAgent significantly improves task success rates, outperforming specialized systems, particularly in complex, multi-step SE tasks across different programming languages. In terms of automating software development using generative AI, the key contribution of HyperAgent is its ability to autonomously handle large-scale, complex coding tasks, including bug fixing, feature addition, and program repair. The system’s use of LLMs across various subtasks showcases how generative AI can enhance automation in SE by reducing the need for manual intervention, especially in navigation, code editing, and execution. However, the paper also highlights several challenges, such as ensuring scalability across different programming environments and managing the computational cost of multi-agent coordination. Limitations include the potential for performance bottlenecks when handling larger codebases and debugging complex issues in real-time environments. Future work proposed in the paper involves integrating HyperAgent with version control systems, enhancing its explainability, and further refining the system to handle more specialized SE domains like security and performance optimization. These improvements could extend its applicability and make it a more practical tool for real-world software development.
\citep{xia2024agentless} challenges the need for complex, autonomous software engineering agents by introducing a simplified approach called AGENTLESS. This approach automates software development tasks, such as bug fixing, using a two-phase process: localization and repair. Unlike existing agent-based systems, which involve complex tool integration and autonomous decision-making, AGENTLESS employs a more straightforward hierarchical process for fault localization followed by patch generation. The paper demonstrates that this agentless approach can solve repository-level software issues with greater cost efficiency and competitive performance compared to state-of-the-art agent-based methods, achieving the highest performance on the SWE-bench Lite benchmark (27.33\%) at a fraction of the cost. Contribution to automating software development using generative AI: AGENTLESS leverages large language models (LLMs) to effectively automate bug localization and repair, offering a simpler yet robust alternative to more complex autonomous agents in software development. By removing the need for intricate tool management and decision-making mechanisms, the approach reduces complexity and improves interpretability. Challenges and Limitations: While AGENTLESS outperforms many open-source approaches, the paper identifies limitations such as reduced performance in scenarios where no localization clues are provided and difficulties in solving problems that require advanced reasoning or complex planning. Additionally, it highlights the need for improved re-ranking and selection techniques to maximize its repair capabilities. Future Work: The authors propose extending the AGENTLESS framework to address more complex software engineering tasks and to improve its problem-solving capabilities through better integration with testing frameworks and enhanced patch selection mechanisms. The paper contributes to the discourse on automating software development by emphasizing the potential of simpler, interpretable AI-driven methods over more complex autonomous agents.

\subsection{Code Generation}
\citep{gu2023effectiveness} provides a detailed empirical study on how large language models (LLMs) like ChatGPT, CodeLlama, and PolyCoder perform in domain-specific code generation tasks, focusing on the fields of web and game development. The authors reveal that while LLMs have shown great success in general-purpose code generation, their performance in domain-specific scenarios degrades significantly. This is largely due to the limited proficiency of these models in handling domain-specific libraries and APIs, resulting in issues such as API misuse and missing API calls. To address these challenges, the paper proposes DomCoder, a novel approach that integrates domain knowledge into LLMs through API recommendations and chain-of-thought prompting strategies. DomCoder shows improved performance across various domain-specific benchmarks, demonstrating the importance of enhancing LLMs with domain-specific prompts and fine-tuning for better results. 
Contribution to Automating Software Development using Generative AI: The paper's key contribution lies in showing how generative AI, when fine-tuned with domain-specific knowledge, can improve the automation of software development tasks, particularly in highly specialized domains such as game and web development. The integration of API knowledge into LLMs significantly enhances code generation performance, suggesting practical applications for automating more complex and specialized software engineering tasks. 
Challenges and Limitations: One major limitation is the scarcity of domain-specific data, which impacts the LLMs’ ability to fully learn the intricacies of domain-specific libraries. Additionally, integrating domain knowledge through complex APIs and prompts increases the difficulty of maintaining consistency and correctness in the generated code. 
Future Work: The authors propose future research directions, including improving LLM training with a richer variety of domain-specific datasets and enhancing prompt design mechanisms to further bridge the gap between general-purpose LLMs and domain-specific requirements. They also suggest exploring more sophisticated knowledge integration techniques, such as fine-tuning models with domain-relevant workflows and patterns to improve performance in complex domains.

\citep{zhang2023planning} introduces a novel approach called Planning-Guided Transformer Decoding (PG-TD), which improves the performance of large language models (LLMs) in code generation tasks by integrating a planning algorithm with Transformer models. Unlike traditional sampling and beam search methods, which rely on generating code first and then evaluating it, PG-TD incorporates a lookahead search that allows the model to make informed decisions during the generation process. This approach enables the model to generate higher-quality programs by considering test case results while the code is being generated. The method significantly improves pass rates on public competitive programming benchmarks compared to baseline methods.
Contribution to automating software development using generative AI: The introduction of PG-TD contributes to automating software development by optimizing code generation and reducing the need for extensive post-generation evaluation. It provides a more efficient way of generating programs that pass more test cases and is model-agnostic, meaning it can work with various Transformer-based LLMs without needing additional data or fine-tuning. 
Challenges and limitations: One of the key challenges of this approach is its reliance on available test cases for evaluating the quality of generated programs. The method is also more computationally expensive than simpler Transformer-based approaches due to the iterative tree search mechanism. Additionally, while it shows clear improvements in competitive programming scenarios, its effectiveness in broader software development contexts has not been fully explored. Future work: The authors propose improving the computational efficiency of PG-TD by exploring parallel tree search techniques and incorporating neural value functions to estimate pass rates more effectively. They also suggest extending the framework to support automatically generated test cases, addressing the issue of missing test cases in real-world scenarios. This paper makes a significant contribution to the ongoing development of generative AI in software engineering by enhancing the accuracy and efficiency of LLM-driven code generation.

\subsection{Knowledge Gaps}

\begin{description} 
   \item[Lack of Domain Knowledge] 
   \item[Hallucination] 
\end{description}

==> Backup/react_code_structure.tex <==
referring to different sections of a React JSX script as "code blocks" is understandable, but in React and software engineering terminology, these sections are typically called "code sections", "declarations", or more specifically by their respective roles. Here are the appropriate terms for each part:

Import Statements – This section at the top of the file imports necessary dependencies, such as React, third-party libraries, or custom components.
State and Variable Declarations – These include React state variables (e.g., useState), refs (useRef), and context variables (useContext) that manage data within the component.
Event Handler Functions – Functions defined within the component that handle events such as user interactions (e.g., onClick, onChange).
Effect Hooks and Lifecycle Methods – Side effects (e.g., API calls, subscriptions) are managed within useEffect in functional components or componentDidMount, componentDidUpdate, and componentWillUnmount in class components.
JSX Return Block (Render Logic) – The rendered UI structure, typically within the return() statement in functional components or the render() method in class components.
Custom Hooks or Utility Functions – If the component includes custom logic for reusability, it may contain custom hooks or helper functions.
Software Engineering Term
The most precise term to describe these functionally distinct sections within a React JSX file is "logical sections" or "concerns". A more structured term based on Separation of Concerns (SoC) would be "functional concerns" in a React component.

However, when discussing different code sections in a single file, a widely accepted term is "component structure" or "React component composition", referring to the way code is organized within a React component.

Instead of "code blocks", you may refer to them as:

Logical sections of a React component
Functional concerns in a React file
Component structure in JSX
React composition pattern
Would you like me to refine this further for a specific use case?

==> Sections/00_AAid.tex <==
This research presents a system-based approach to automate the software development of sophisticated GIS-based web applications to facilitate the urban and environmental management in smart city research, using ontology-driven prompts and ChatGPT, a widely used large language model (LLM). Our approach aims to leverage the AI model's generative, reasoning, and learning capability to create a primitive autonomous agent that helps academia researchers and would-be developers lower the technical barrier and cost to developing cyberinfrastructure and scientific software tools. At the technical level, we implemented a prototyping framework that employ a Knowledge Graph (KG) as the digital representation of software engineering practices, popular application stacks, and domain science knowledge to generate, tune, and enhance the engineered prompts through iterative procedures, creating accurate instructions to guide ChatGPT 4.0 API and LangChain to automate the development of a web-based geo-visual dashboards using widely-used frameworks and technologies favored by the industry. We demonstrate the performance and feasibility of our framework through a case of an AI-generated web applications. Through this study, we explore the LLM's potential as a full-stack web developer and GIS analyst trained by scientific knowledge graph to utilize advanced software design and architecture patterns (e.g., MVC and MVVM) and complex scientific data () to produce robust web app on both the server- and client-side. 

==> Sections/backup/1_Intro.tex <==
\section{Introduction}
\label{Introduction}
Over the past decades, scientific web applications (Web Apps), such as CyberGIS systems, visual analytics dashboards, digital twin platforms, and online decision support systems, have become indispensable tools for both the scientific community and the public to discover, query, visualize, and download vast urban and environmental data sets for smart city research \citep{ferre2022adoption, dembski2020urban}. Aligned with the NSF's cyberinfrastructure (CI) initiative, academia and government agencies have increasingly adopted these applications as part of interdisciplinary informatics projects, providing effective, user-friendly tools for data dissemination \citep{yu2021coevolution}. With advances in internet and communication technologies, computing hardware, and artificial intelligence, these tools are transforming urban and environmental research by enabling data- and simulation-driven insights for decision support \citep{kadupitige2022enhancing}, fostering collaborative research through data and simulation integration \citep{parashar2019virtual} and enhancing education and public engagement in citizen science and voluntary data collection \citep{skarlatidou2019volunteers}. Key application areas include water resource management \citep{souffront2018cyberinfrastructure, xu2022overview}, hazard mitigation \citep{mandal2024prime, xu2020web, garg2018cloud}, intelligent transportation systems \citep{xu2023smart, xu2022interactive, ghosh2017intelligent}, connected and automated vehicles \citep{xu2023mobile, kampmann2019dynamic}, built-environment and building energy management \citep{jia2019adopting, kim2022design, xu2022geo}, pandemic management \citep{xu2021episemblevis, li2021emerging, thakur2020covid}, and urban planning and design \citep{alatalo2017two}. Numerous interdisciplinary studies highlight the transformative potential of these web applications in advancing environmental and urban research, as well as smart city management. Their ongoing evolution is driven by the integration of emerging technologies like artificial intelligence, the Internet of Things (IoT), edge computing, and cyber-physical systems.

Despite advancements in scientific web applications, developing customized tools like cyberGIS and digital twin platforms for integrating and visualizing diverse environmental or urban data (e.g., hydrological, traffic flow, meteorological data, or simulations) remains highly demanding and resource-intensive \citep{shanjun2024design, siddiqui2024digital, lei2023challenges}. These efforts require expertise in software and data engineering, as well as time-consuming tasks like client-server development, database management, real-time analytics, machine learning, and simulations \citep{ikegwu2022big}. Consequently, researchers often shift from their core scientific work to learn complex web programming, UI/UX design, and database technologies \citep{li2022bibliometric}. Although modern software practices like design patterns aim to streamline development, their effective use demands specialized software engineering knowledge \citep{fayad2015software}. Researchers with data analytics expertise often lack formal software development experience, facing challenges even when skilled engineers are involved \citep{kim2017data}. Designing, deploying, and maintaining large-scale web apps remains labor-intensive, limiting scalability and adaptability in platforms like cyberGIS or digital twins \citep{shah2024optimizing, mcbreen2002software, liu2015cybergis}. Emerging Generative AI (GenAI) technologies offer potential to automate web development for environmental and urban research. While studies have shown the feasibility of training large language models (LLMs) like GPT for automating data analytics and development tasks \citep{liang2024can, liukko2024chatgpt}, challenges remain for complex scientific web apps due to inefficiencies in prompting methods, limitations in domain knowledge, and LLMs' attention mechanisms, which are trained on generalized text data.

\begin{figure*}[htb]
 \centering
\includegraphics[width=\textwidth]{Figures/Figure_1.png}
 \caption{From annotated wireframe to code generation, a knowledge driven framework for automated software development of cyberGIS platform for visualizing time-series and spatial data. }
 \label{fig:concepts}
\end{figure*}

This paper introduces a knowledge-augmented code generation framework that integrates software engineering best practices, domain expertise, and advanced software stacks to enhance Generative Pre-trained Transformers (GPT) for front-end development. The framework automates the generation of GIS-based web applications, including visualization dashboards and analytical interfaces, directly from user-defined UI wireframes created in tools like PowerPoint or Adobe Illustrator. It leverages industry-standard web frameworks and software engineering best practices to ensure scalability, maintainability, and efficiency. We propose a novel context-Aware visual prompting method, implemented in Python, that interprets wireframes to extract layout structures and interface elements, enabling LLMs to generate front-end code while incorporating both software engineering principles and domain knowledge through Chain-of-Thought (CoT) and Retrieval-Augmented Generation (RAG) paradigms. A case study demonstrates the framework’s capability to autonomously generate a modular and maintainable web platform hosting multiple dashboards for visualizing and interacting with environmental and energy data, including time-series data sets, GIS shapefiles, and raster imagery, based on user-sketched wireframes. By leveraging a knowledge-driven approach, the framework ensures that the generated front-end code adheres to industry-standard software design and architectural patterns, including the React framework and Model-View-ViewModel (MVVM) architecture, facilitating long-term scalability and maintainability. This approach significantly reduces manual effort in UI/UX design, coding, and maintenance, pioneering a scalable, autonomous, and robust solution for developing web applications that support smart city advancements.


%While AI tools cannot yet fully replace the need for human oversight in creating complex systems, they can significantly reduce the effort required for coding, optimizing workflows, and applying best practices in software engineering. By automating routine and repetitive development tasks, generative AI offers the potential to make scientific web application development more efficient, accessible, and scalable, allowing researchers to focus on their primary scientific objectives while ensuring the platforms they rely on are robust and maintainable.

 



%These software tools offer integrated access to diverse data and simulation results, facilitating data-driven decision-making across various urban disciplines, including 
%\citep{}. 


%The development efforts for creating scientific software tools, such as web-based visualization and visual analytics dashboard, online digital twin platforms, and cyberinfrastructure, are critical to facilitate environmental and urban research from multiple aspects. These aspects include 


 




 


%By integrating real-time data with user-friendly and user-intuitive interfaces, as well as interactive visualizations, they empower users to explore complex systems, generate insights, and develop solutions for urban and environmental challenges \citep{}. 

%urban digital twin platform or a cyberinfrastructure, are often time-consuming and labor-intensive, requiring seamless collaboration and effective communication between both the domain science experts and experiences software engineers and programmers. To reduce the technical barriers for domain scientists to develop advanced urban digital twins for research applications, we propose an autonomous software development solution by leveraging the domain-knowledge representation capability of scientific ontologies, in combination with the generative AI capability of Large Language Models (LLMs), such as the ChatGPT, for automated software implementation (e.g., design and architecture patterns using MCV paradigms, code generation, automated dev/ops using Dockers and Kubernetes).

%Large Language Models have revolutionized fields ranging from creative writing to code generation with their deep understanding of human language. In this paper, we harness these capabilities to automate the development of digital twin platforms for smart city research and management. Integrating LLMs with software engineering paradigms and scientific ontologies, we introduce an autonomous pipeline for prototyping digital twins. This pipeline leverages urban science domain ontologies to transform scientific concepts (datasets, simulation models, metrics, AI algorithms) into software components using robust design patterns. Utilizing LLMs for natural language understanding, reasoning, and coding, it automatically implements these components in popular programming languages. Our AI-powered urban digital twins offer advanced capabilities: real-time IoT data visualization, multi-objective decision optimization, and predictive analytics for urban dynamics. We validate our pipeline with three smart city case studies focusing on freight transportation management, urban climate modeling, and building energy optimization. Implemented using the GPT-4 API in a Python environment, our pipeline synergizes with knowledge graphs created using prevalent ontology languages. The results are compelling: for each case study, the pipeline efficiently generated operational digital twins using an MVC-based Python framework. This marks a significant reduction in manual software design and coding efforts. Our research presents a pioneering path towards next-generation AI-powered urban digital twins that are self-generating, self-organizing, and self-executing, demonstrating the transformative potential of LLMs in urban technology development.

==> Sections/backup/2_Literature.tex <==
\section{Literature Review}
\label{Literature Review}
In recent years, the rise of LLMs like GPT-3 \citep{brown2020language}, GPT-4 \citep{sun2023gpt}, and the emerging DeepSeek model has introduced new possibilities for revolutionizing software development through autonomous code generation \citep{guo2024deepseek}. LLMs have demonstrated a remarkable ability to understand and generate human language, enabling them to perform a wide range of tasks, including reasoning, code generation, and problem-solving \citep{li2023autonomous, tupayachi2024towards}. By integrating LLMs with RAG techniques, developers can enhance these models' capacity to retrieve and incorporate domain-specific knowledge, improving the accuracy and reliability of generated code. This combination holds the potential to automate significant portions of the software development process, such as requirement definition, bug fixing, feature implementation, and program repair, while reducing the need for manual intervention. As a result, LLMs and RAG are poised to fundamentally transform how software is developed for specific applications, offering a path toward more efficient and scalable solutions for both routine and complex coding tasks \citep{meyer2023llm, baldazzi2023fine}.

\subsection{A Review of LLM-Based Approaches in Software Development}
The applications of LLMs in software engineering and code generation are diverse and rapidly expanding. The following subsections review various aspects of their use in software engineering tasks. This paper specifically focuses on evaluating the capability of LLMs in web application development.

\subsubsection{Automating Software Engineering Tasks}
A few studies have conducted reviews and proposed potential opportunities and challenges for adopting LLMs to facilitate various software engineering tasks. \citet{hou2023large} offers a comprehensive review of how LLMs are applied in software engineering, categorizing them into architectures like encoder-only, encoder-decoder, and decoder-only models. The growing use of decoder-only models (e.g., GPT) is highlighted for automating tasks like code generation and completion, significantly reducing manual coding effort. However, key challenges remain, including handling domain-specific knowledge, improving data set quality, and addressing the complexity of SE tasks that go beyond simple text generation. Notably, the need for better data prepossessing, model fine-tuning for specific SE tasks, and inclusion of more diverse data sets, especially from industrial contexts, are underscored, which are often underrepresented. Data set variety, enhancing LLM robustness for complex SE tasks, and refining evaluation metrics are noted necessary steps for better assessing LLMs in real-world scenarios. LLMs are increasing recognized with growing potential to assist in SE, however, these models are not yet capable of fully replacing human developers in more intricate processes. 

\citet{phan2024hyperagent} introduces HyperAgent, a multi-agent system designed to address various software engineering (SE) tasks using specialized agents like Planner, Navigator, Code Editor, and Executor. Evaluated on benchmarks, such as SWE-Bench and Defects4J, HyperAgent excels in GitHub issue resolution, repository-level code generation, and fault localization, outperform specialized systems in complex, multi-step tasks. Its key contribution lies in automating large-scale coding tasks (e.g., bug fixing, feature addition) using LLMs, reducing the need for manual intervention across planning, code editing, and execution. However, challenges include scalability across diverse programming environments, and high computational cost of multi-agent coordination. Future work is expected to integrate version control systems, improve explainability, and extend the system to specialized SE domains like security and performance optimization, making HyperAgent a more practical tool for real-world development.

\citet{xia2024agentless} introduces AGENTLESS, a simplified approach that automates SE tasks like bug fixing through a two-phase process: localization and repair. Unlike agent-based systems, AGENTLESS employs a hierarchical structure that eliminates complex tool integration, achieving superior cost efficiency and competitive performance, notably achieving 27.33\% on the SWE-bench Lite benchmark. LLMs are demonstrated to effectively automate bug localization and repair without the complexity of autonomous agents. However, this approach faces challenges in scenarios without localization clues and in tasks requiring advanced reasoning. It is acknowledged that future work should expand AGENTLESS to more complex SE tasks, improve patch selection, and integrate testing frameworks, offering a simpler and more interpretable alternative to complex agent systems for automating software development.

\subsubsection{Evaluating LLM for Software Development}
With the rise of generative AI applications, several studies have conducted comprehensive reviews and evaluations on the feasibility of various LLMs for code generation and more complex software development tasks.
  
\citet{liang2024can} explores the potential of GPT-4 to replicate empirical software engineering research by generating code for analysis pipelines. Through a user study involving 14 participants and seven empirical SE papers, the study found that while GPT-4 surfaced correct assumptions and generated high-level analysis plans, it often lacked domain-specific expertise. The generated code frequently contained errors, such as incorrect data sources and missing steps, with only 30\% being executable without modification. Despite these limitations, GPT-4 shows promise in automating parts of the SE process, particularly in replicating studies and structuring analysis code, though human oversight remains critical for correcting errors and ensuring accuracy. \citet{sandberg2024evaluating} investigates GPT-4’s ability to automate full-stack web application development, assessing key metrics like prompt efficiency, debugging effort, and code quality. The study reveals that GPT-4 excels at generating functional applications for simpler projects, significantly speeding up development. However, as complexity increases, GPT-4 struggles with debugging, integration, and complex logic, requiring substantial human intervention. While the tool effectively generates foundational code, it falls short in handling intricate systems, underscoring the need for human expertise in ensuring quality and reliability in complex software development.
\citet{gu2023effectiveness} presents an empirical study on how LLMs like ChatGPT, CodeLlama, and PolyCoder perform in domain-specific code generation, particularly in web and game development. The study reveals that LLMs struggle with domain-specific libraries and APIs, leading to issues like API misuse. To address this, the authors propose DomCoder, a model that integrates API recommendations and chain-of-thought prompting, significantly improving performance in domain-specific tasks. The key contribution is demonstrating how fine-tuning LLMs with domain-specific knowledge can enhance automation in specialized software development tasks. However, challenges include the scarcity of domain-specific data and the difficulty of maintaining consistency in API integration. Future work involves enriching training data sets and refining prompt design to bridge the gap between general-purpose LLMs and domain-specific requirements.
\citet{fan2023large} provides an in-depth review of LLMs like GPT, BERT, and Codex, focusing on their integration into software engineering tasks such as code generation, program repair, and automated testing. This work showcases LLMs' ability to revolutionize software development by automating tasks like code completion and bug detection, thereby enhancing developer productivity and efficiency. Several challenges are identified, including LLMs' tendency to hallucinate (generate incorrect but plausible outputs), struggles with domain-specific tasks, and the need for fine-tuning models for specialized contexts. It also highlights the issue of non-deterministic outputs, complicating scientific evaluation, and the oracle problem in verifying the correctness of generated solutions. Improving prompt engineering, hybridizing LLMs with traditional SE methods, and exploring their application to less-studied areas like requirements engineering and software design are suggested as areas of advancements. Integrating automated testing with LLM outputs is proposed as a means to mitigate hallucination and enhance reliability. The paper’s novelty lies in its exploration of LLM integration into SE tasks, while acknowledging the persistent challenges in ensuring the reliability and correctness of these models.

\subsubsection{Code Generation}
Several ongoing research efforts have explored LLM-based approaches to facilitate code generation. \citet{guo2024deepseek} introduced DeepSeek-Coder, a significant advancement in code-focused LLMs that addresses the limitations of closed-source models by offering a high-performance, open-source alternative. DeepSeek-Coder comprises models ranging from 1.3B to 33B parameters, trained on 2 trillion tokens spanning 87 programming languages. Unlike traditional code models, it leverages repository-level data construction to enhance cross-file understanding, improving its ability to generate coherent and structured code. Additionally, it incorporates a Fill-in-the-Middle (FIM) training approach and supports a 16K context window, enabling it to handle complex coding tasks more effectively. Benchmark evaluations demonstrate that DeepSeek-Coder outperforms leading open-source models, such as CodeLlama and StarCoder, and in some cases even exceeds OpenAI’s GPT-3.5 Turbo in code generation tasks. By offering a permissive license, DeepSeek-Coder empowers researchers and developers to explore its potential in autonomous code generation, software development, and problem-solving, further narrowing the gap between open-source and proprietary code models. \citet{zhang2023planning} introduces Planning-Guided Transformer Decoding (PG-TD), a novel approach that integrates a planning algorithm with Transformer models to improve code generation by considering test case results during the generation process. This method outperforms traditional sampling and beam search methods, increasing pass rates on competitive programming benchmarks. The key contribution is the optimization of LLM-driven code generation by reducing post-generation evaluation, making the approach model-agnostic. However, PG-TD is computationally expensive and relies on available test cases, limiting its application in broader software development contexts. Future work aims to improve computational efficiency through parallel tree search techniques and extend the method to automatically generate test cases, enhancing its applicability to real-world software development.

In the GIS sector, \citet{hou2024can} examines the limitations of general-purpose LLMs in geospatial code generation and proposes strategies for improvement. Due to a lack of domain-specific training, LLMs generate inaccurate and inefficient geospatial code, leading to issues like coding hallucinations, deprecated functions, incompatible dependencies, and incorrect parameters. They also struggle with multi-modal geospatial data (e.g., raster, vector, elevation models) and complex spatial operations, failing to recognize built-in GIS functions in platforms like Google Earth Engine, OpenLayers, and Leaflet. Even advanced prompting techniques offer only marginal improvements, exposing fundamental training deficiencies. To address this issue, the study introduces GeoCode-Eval (GCE), an evaluation framework assessing LLMs' cognition, comprehension, and innovation in geospatial programming. Systematic testing reveals significant shortcomings across commercial and open-source LLMs. The authors propose fine-tuning with domain-specific datasets, demonstrated by GEECode-GPT, a Code LLaMA-7B model trained on Google Earth Engine scripts, which significantly improves execution accuracy. Additionally, they introduce GeoCode-Bench, a benchmark data set evaluating LLMs through multiple-choice, fill-in-the-blank, and coding tasks. The study also advocates instruction-tuning using NASA Earth Data, USGS, and OpenStreetMap to further enhance geospatial reasoning. In conclusion, the study highlights LLMs' current limitations in geospatial programming and presents fine-tuning, benchmarking, and instruction-tuning as key solutions to bridge the gap, improving their reliability and usability for geospatial applications.

\subsubsection{Front-end App Development from UI Prototypes}
\citet{xiao2024prototype2code} introduces Prototype2Code, an end-to-end framework for automating front-end code generation from UI design prototypes. Traditional UI-to-code methods often produce fragmented elements and unstructured code, leading to poor maintainability. To address this, Prototype2Code integrates design linting, graph-based UI structuring, and LLMs to enhance code generation. The framework first detects and corrects UI inconsistencies through linting, then constructs a hierarchical layout tree for structured component relationships. A Graph Neural Network (GNN)-based classifier refines UI elements before LLMs generate modular HTML and CSS code. Comparisons with tools like CodeFun and GPT-4V-based Screenshot-to-Code demonstrate superior visual fidelity, readability, and maintainability, validated through SSIM, PSNR, and MSE metrics. A user study confirms Prototype2Code reduces manual modifications while improving usability and production readiness. By incorporating design intelligence and AI-driven automation, it streamlines front-end development and minimizes human intervention. Future work aims to support dynamic components, interactive behaviors, and cross-platform adaptability.

\citet{manuardi2024images} explores AI-driven front-end automation by converting UI mockups into structured code. While tools like GitHub Copilot enhance text-based programming, they struggle with UI-driven development, where visual design is central. The study proposes a multi-modal AI system combining computer vision and LLMs to bridge this gap. It processes UI images through edge detection, contour analysis, and OCR, generating a standardized intermediate representation. A multi-modal LLM then translates this into front-end code, tailored for frameworks like Angular and Bootstrap. Implemented as a web-based tool at Blue Reply, the system improves development efficiency by reducing manual coding while ensuring maintainability. By integrating computer vision and AI-powered code generation, this approach advances automated, intuitive front-end development.

\subsection{Limitation and Knowledge Gaps}
Despite significant advancements in LLM-powered code generation for software development, several limitations and knowledge gaps persist, particularly in scientific applications and GIS-based web applications. These challenges hinder the seamless automation of both front-end and back-end development, underscoring the need for further research and innovation. The key challenges are outlined below, labeled C1 to C4 for reference in later discussions.

\begin{description} 
   \item[C1. Limited Graphical and Visual Prompting Techniques:] Current LLMs primarily rely on text-based prompting, which limits their ability to interpret graphical user interface (GUI) designs and wireframe sketches effectively. Although visual prompting techniques, such as image-to-code models, have shown potential, they often struggle with complex UI layouts, interactive components, and contextual relationships between elements. The lack of robust graph-based UI understanding restricts the ability of LLMs to accurately generate structured, modular front-end code from visual design prototypes.

    \item[C2. Lack of Software Engineering Practices in AI-generated Codes:] 
    LLM-generated front-end code often consists of plain HTML and JavaScript, lacking integration with software engineering design principles and architectural patterns such as MVC and MVVM, which are widely used in the IT industry to enhance code readability and maintainability \citep{xiao2024prototype2code}. While AI-assisted programming tools can generate functional snippets, they frequently neglect design patterns, coding conventions, and software architecture best practices, resulting in code that is challenging to maintain in production \citep{ghoshdesign, nguyen2023generative}. Additionally, current LLM-driven development workflows rarely incorporate continuous integration/continuous deployment (CI/CD) pipelines, software testing frameworks, or version control systems, limiting their practical usability in large-scale software development \citep{corona2025question, mendoza2024development}.
   
   \item[C3. Lack of Domain Knowledge for Developing GIS and Scientific Applications] 
   General-purpose LLMs lack deep expertise in GIS and scientific computing, resulting in suboptimal performance when generating domain-specific software \citep{zhang2024bb, mansourian2024chatgeoai}. Developing GIS-based web applications requires expertise in geospatial data processing, web-based mapping engines, web map server applications, and data visualization libraries, along with interoperability with standards such as GeoJSON, WMS, WFS, and 3D point clouds \citep{xu2024semi, xu2019web, berres2021multiscale}. These interdisciplinary aspects bridge GIS, data science, and software engineering, creating challenges for general-purpose LLMs, which often struggle due to insufficient training data and lack of domain-specific guidelines \citep{hou2024can}. While recent studies have explored and prototyped fine-tuned LLMs for generating geospatial code to support spatial analysis and GIS problem-solving \citep{hadid2024geoscience, hou2024geocode, akinboyewa2024gis}, they primarily focus on computational GIS tasks. However, generating web-based visual dashboards and CyberGIS software using web programming languages and frameworks remains largely unexplored, leaving a critical gap in this domain.
 
   \item[C4. Package Management Challenges:] AI-generated code often introduces dependency and package management issues, particularly when working with scientific computing, GIS, and front-end frameworks. LLMs frequently suggest outdated or incompatible packages, mismatched versions, or deprecated functions without considering package conflicts and runtime environments \citep{hou2024can}. In web-based GIS applications, maintaining compatibility between Python, JavaScript, or C++ libraries (e.g., Django, Flask, OpenLayers, Leaflet, Mapbox, PyProj) is crucial, yet current LLM-driven code generation fails to account for such dependencies effectively \citep{mahmoudi2023development}. This results in increased debugging time, compatibility issues, and broken software deployments.
\end{description}

Given these knowledge gaps, there is a need for a robust framework that enables a reliable code generation pipeline for automating the development of front-end GIS web applications in a one-stop-shop manner. This framework should take user-defined GUI sketches, created in common, non-technical software such as PowerPoint, as its sole input, streamlining the development process for users without programming expertise. 

 

==> Sections/backup/3_Method.tex <==
\section{Methodology}
\label{Methdology}
In the following subsections, we first discuss the motivation behind our research, highlighting the challenges we aim to address and presenting our overall strategy and knowledge-driven approach at a conceptual level. Next, we outline the software design requirements for our proposed framework, focusing on target users and key features. With these requirements defined, we introduce the overall framework design, detailing its major steps. We then provide an in-depth discussion of individual steps, including visual contextual prompting techniques, the software engineering and GIS knowledge base built on the RAG paradigm and vector databases, and the final step of code generation using a Knowledge-Augmented Generation (KAG) paradigm through iterative processes. 

Our approach focuses on knowledge augmentation for LLM-driven coding tasks rather than fine-tuning or training specific models. We propose a system-based, adaptable method that integrates software knowledge and engineering practices into user-selected LLMs. Additionally, we introduce a generalizable approach that enables end-users to leverage customly sketched UI wireframes as inputs to prompt LLMs for front-end web application development.

\subsection{Motivation and Contributions}
Our primary motivation is to develop a knowledge-driven approach for instructing LLMs, particularly GPTs, to facilitate automated code generation that aligns with software engineering best practices. This approach aims to support the development of robust and maintainable web-based GIS applications for sharing and visualizing scientific data. By leveraging industrial-grade practices, web frameworks, and modern software stacks, our method seeks to lower technical barriers for aspiring developers—specifically domain scientists with coding experience but limited knowledge of software engineering—enabling them to generate front-end code for cyberGIS software more effectively.

To address the challenges in geospatial code generation identified in recent studies \citep{hou2024can, hou2024geocode}, particularly the limitations of general-purpose GPT models in handling built-in GIS and visualization libraries and managing complex package dependencies, we propose a novel knowledge-driven approach. Existing models frequently exhibit hallucinations, runtime errors, and an inability to generate complex CyberGIS applications with advanced data querying and visualization capabilities \citep{hou2024can}. Our approach seeks to overcome these limitations by integrating structured domain knowledge with intelligent prompt engineering and package management solutions, ensuring that LLM-generated code is accurate, executable, and aligned with industry standards. The key novelties of our contributions are as follows:
\begin{description}
    \item[Knowledge-Augmented Code Generation through Code Base and Knowledge Representations: ] Unlike previous efforts that primarily focus on fine-tuning LLMs or developing knowledge bases for geospatial libraries to enhance geospatial code generation \citep{hou2024can, hou2024gee}, our approach leverages Knowledge-Augmented Generation (KAG) technologies to construct comprehensive code-base and knowledge representations in the form of a knowledge graph. This knowledge graph integrates software engineering principles with existing code examples, incorporating advanced design and architectural patterns into the CyberGIS domain. By embedding structured knowledge and real-world code instances, our approach fosters a more systematic and informed methodology for geospatial application development, improving the accuracy, maintainability, and scalability of LLM-generated geospatial code.
    \item[Visual Contextual Prompting Technique: ] Our visual contextual prompting technique is a Python-based system that enables non-technical users to design web applications using SVG-based wireframes, which are then automatically translated into structured prompts for LLM-driven code generation. This approach allows domain scientists and other non-programmers to create UI layouts in familiar tools like PowerPoint and Adobe Illustrator, which are then processed by our Python program to extract GUI components, spatial relationships, and functional annotations.
    The system queries a visual contextual knowledge base to retrieve technical implementation details for various UI elements, ensuring compatibility with modern frameworks such as React, Angular, Tailwind CSS, Bootstrap, Leaflet, and D3.js. Rather than relying on LLMs to generate raw HTML and JavaScript from scratch, this method leverages structured knowledge representations to provide precise, context-aware prompts that improve code accuracy, maintainability, and adherence to industry best practices. By integrating wireframe-based design interpretation with knowledge-driven prompt engineering, this technique significantly enhances LLM-assisted geospatial and web application development, making it more accessible to non-programmers while ensuring high-quality, scalable code generation.
    
    \item[Software Engineering Practices Implementation: ] We introduce a chain-of-steps guidance framework that utilizes engineered prompts combined with a novel visual contextual prompting technique to instruct LLMs in generating robust, web-based GIS applications. Unlike conventional methods, our approach ensures that LLMs adhere to industry-standard web development frameworks, such as the React framework, which follows the Model-View-ViewModel (MVVM) architecture to build modular and maintainable single-page applications (SPAs) for querying and visualizing GIS data in web browsers. By structuring prompts around well-defined software engineering best practices, we enhance the LLM’s ability to generate high-quality, scalable GIS applications that align with modern web development paradigms.
    \item [Multi-tool Package Management: ] In addition to application generation, we employ a knowledge-driven approach to generate structured commands that guide industry-standard package management tools, such as the NPM (Node Package Manager) for Javascript and Typescript package management, to resolve package dependencies effectively. LLMs often struggle with package compatibility and dependency resolution, leading to outdated or incompatible package suggestions. Instead of relying on the LLM to generate package management files directly—which requires extensive, up-to-date knowledge of package versions—our method abstracts package management and version control at a higher level. By leveraging structured knowledge representations, we enable the LLM to control existing package management tools dynamically, ensuring that dependency resolution is handled efficiently and in alignment with best practices. This approach mitigates the risk of broken deployments and streamlines the software development workflow, making LLM-assisted GIS application development more reliable and maintainable.
\end{description}
In this study, we present the conceptual design of our framework and its technical implementation, developed using Python within a Jupyter Notebook environment. The primary focus of our research is to explore and experiment with new paradigms that enhance existing LLM-driven code generation efforts. Rather than being tailored to a specific LLM model, our approach is designed as a generalizable knowledge framework that can accommodate and integrate with various GPT-based models, ensuring flexibility, adaptability, and scalability across different AI-driven coding workflows.

\subsection{Design Requirements}
\label{subsec:DesignRequire}
The target users of our proposed framework are domain scientists with strong scientific computing and programming skills in geospatial analysis, simulations, and data modeling. However, they have limited or no exposure to software engineering principles and best practices for developing modular, maintainable front-end web applications using widely adopted software stacks and technologies in the IT industry.

The detailed technical design requirements of our proposed framework are as follows:
\begin{description}
    \item[R1. Support for UI Sketches and Wireframes as Inputs:]  
    The framework should accept UI sketches and wireframes as input, allowing users to visually define the structure and layout of their web applications without requiring extensive front-end development or cyberGIS expertise.
    
    \item[R2. Minimal UI/UX Expertise Required for Wireframing:]  
    Users should be able to create wireframes with minimal UI/UX design experience, ensuring accessibility for domain scientists without specialized front-end design skills. The framework should accept wireframes casually sketched using commonly available software, such as vector graphics created in Microsoft PowerPoint or Word, rather than requiring professional UI/UX prototyping tools like Adobe XD, Figma, or the discontinued Adobe Muse.
    
    \item[R3. Modular and Extensible Knowledge Base:]  
    The framework should provide a structured and expandable knowledge base that allows developers and open-source communities to incrementally refine and customize sample code. By integrating domain-specific and software engineering knowledge, the framework can enhance its ability to generate front-end code with advanced features while leveraging the latest code libraries—all while adhering to best practices.
    
    \item[R4. Integration of Software Engineering Practices:]  
    The system should incorporate established software design and architectural patterns to enhance code maintainability, scalability, and compliance with industry standards. For instance, modern web applications are rarely built using plain HTML, JavaScript, and a basic Python web server. As applications grow in complexity—integrating more features, data, and user workflows—it becomes essential to adopt software engineering best practices, such as Separation of Concerns (SoC) and the Singleton design pattern. These principles help modularize components, optimize performance, and promote code reusability, ultimately leading to the development of robust web frameworks that abstract these practices into MVC (Model-View-Controller) and MVVM (Model-View-ViewModel) architectures. We aim to develop a systematic approach to guide existing LLMs specialized in code generation for specific domain areas, ensuring they adhere to IT industry conventions and technologies (e.g., web frameworks like React) to generate robust and scalable front-end web applications.
    
    \item[R5. Multi-tool Paradigm for Package Management:]  
    A multi-tool approach should be employed to manage software dependencies, leveraging dedicated package management and versioning tools specific to each programming language (e.g., Conda for Python environments and NPM or NVM (Node Version Manager) for server-side JavaScript and TypeScript). This ensures robust package selection, version control, dependency management, and seamless integration of external libraries.
    
    \item[R6. Ease of Deployment and Execution:]  
    The generated applications should be easy to deploy and execute, minimizing the technical complexity required for setting up and running the resulting web-based GIS software. 
\end{description}
Based on these design requirements, we developed a comprehensive framework within a Python environment enabled through Jupyter Notebook. This framework enables the deployment of a code generation pipeline that produces a front-end codebase in a local file-based system. The choice of a Python Jupyter environment is justified by Python’s widespread use in GIS-related tasks, with many major spatial analysis libraries built in Python. More importantly, Python seamlessly integrates with APIs and platforms for both commercial and open-source LLMs, such as OpenAI's ChatGPT API and Ollama, a framework for running local LLMs.

\subsection{Framework Design}
\label{subsec:frameworkDesign}
The overall framework design is illustrated in Figure \ref{fig:arch}, where we define 12 tasks (T1–T12) categorized into three major steps that form the core of the code generation workflow. These steps include: (1) Visual Contextual Prompting, (2) Knowledge Base and Code Base, and (3) Knowledge-Augmented Code Generation. The framework takes as input one or more user-defined wireframes that specify the layout and features of the GUI across different pages. As output, it generates the complete code base for a React project.

\begin{figure*}[htbp]
 \centering
\includegraphics[width=\textwidth]{Figures/Figure_Overall_Framework.pdf}
 \caption{Overall framework architecture.}
 \label{fig:arch}
\end{figure*}

\subsubsection{Visual Contextual Prompting}
\label{subsec:simulations1}
In Step 1, we introduce a novel visual contextual prompting technique implemented using Python scripts. This technique parses, interprets, and translates GUI wireframes into structured prompts that guide LLMs in generating high-quality JavaScript and TypeScript code. Unlike conventional prompting methods that rely solely on textual descriptions, our approach empowers non-technical users, such as domain scientists, to design web applications visually using familiar sketching tools like PowerPoint and Adobe Illustrator.

Many existing graphical prompting methods rely on computer vision (CV)-based techniques to interpret wireframes from bitmap images such as PNG and JPEG. In contrast, our method takes a different approach by processing wireframes in SVG format, which is more easily editable and modifiable during the prototyping stage. This provides a structured yet flexible way to define user interface (UI) components without requiring programming expertise. This step consists of two tasks, T1 and T2, designed to meet the design requirements R1 and R2 outlined in Subsection \ref{subsec:DesignRequire}. The details of these tasks are as follows:
\begin{description}
    \item[T1. Vectorization \& Content Interpretation] A Python program has been developed to process wireframe files exported from PowerPoint or Adobe Illustrator in vector formats (e.g., EPS, SVG). The program extracts spatial and contextual information from graphical elements stored in these vector files to construct the HTML layout and components. Each GUI component—such as dropdown menus, web maps, charts, and form inputs—is represented as a vector graphical entity with embedded annotations that define its intended functionality and attributes. These annotations specify critical details, including whether a component functions as a data visualization element (e.g., bar chart, pie chart), a mapping interface (e.g., web map, layer switcher), or a UI control (e.g., button, slider, dropdown menu). Additionally, the annotations capture interactions and dependencies between components, which are later utilized to generate prompts instructing LLMs on how to bind events to these elements.
    \item[T2. Visual Contextual Info Calculation]  Another script is developed to calculate the visual contextual information of each SVG element, which represent individual HTML element in the GUI. The contextual information is used to describe the position, size, and style of each HTML element, and is later combined with the extracted wireframe annotations to create engineered prompts that provide LLMs with precise, context-aware instructions. These prompts not only define the individual components but also establish their interdependencies, layout structures, and event handling logic within the larger web application architecture. This structured approach significantly improves the accuracy, efficiency, and maintainability of LLM-generated code, ensuring that outputs conform to industry standards while preserving the original design intent of the non-technical user. By integrating visual design with contextual knowledge-based prompting, this technique effectively lowers the barrier for domain scientists and other non-programmers to develop sophisticated, web-based GIS and data visualization applications without requiring direct coding expertise. 

\subsubsection{Knowledge Base and Code Base}
\label{subsec:KB_CB}
The input information, including graphical components, visual contextual details, and annotations extracted from user-defined wireframe files, captures only the GUI design and software requirements. These specifications are expressed in plain, non-technical language, enabling users without web development or computer science expertise to define their application requirements without coding knowledge. In this setting, a combined knowledge base and code base is required to interpret plain-language inputs from context-aware visual prompts and annotations, transforming them into software development strategies. These strategies facilitate the generation of structured prompts enriched with sample code, which are then used to guide LLMs for code generation in a Retrieval-Augmented Generation (RAG) framework. 

Our knowledge base was developed by constructing knowledge graphs that encapsulate software development experiences, system requirements, and architectural designs derived from our previous projects on digital twins, cyber infrastructure, and web-based visual analytics dashboards, as depicted in Table \ref{tab:KG_previousProjects}. These knowledge graphs document and classify software stacks, componentization methods, and system designs based on domain-specific use cases and data types. 

\input{Table/table1.tex}

An example of the knowledge graph structure is depicted in Figure \ref{fig:example}. The sample code stored within these graphs is either excerpted and refined from previous projects or augmented using the ChatGPT API under expert review and supervision.

The process of knowledge-driven prompting follows a procedural approach, structured through tasks T3 to T8, ensuring a systematic and context-driven software development workflow. These tasks are detailed in the following list, with their rationale depicted in Figure \ref{fig:KG_method}. 

\begin{figure*}[htbp]
 \centering
\includegraphics[width=\textwidth]{Figures/Figure_knowledge_base.pdf}
 \caption{Structured knowledge representations for translating plain-language annotations from UI wireframes into structured prompts using technical language. }
 \label{fig:KG_method}
\end{figure*}

\begin{description}
    \item[T3. Define Framework \& Library Selection Criteria]  
    This task establishes criteria for selecting web frameworks and libraries based on wireframe annotations. A vector index search on a knowledge graph—spanning software engineering and CyberGIS domains—maps user-defined UI elements (e.g., date selector, GIS map) to corresponding React components (e.g., calendar dropdown, web map engine). The knowledge graph stores metadata on HTML elements, events, and best practices, ensuring context-aware and industry-aligned component selection.

    \item[T4. Generate HTML/TypeScript Component Tree]  
    Using extracted GUI components and annotations, this task constructs a structured HTML/TypeScript component tree representing the front-end layout. Components are mapped to web elements while preserving semantic correctness, hierarchical relationships, and relevant CSS styles. Wireframe context guides nested structures and component interactions.

    \item[T5. Classify \& Select Front-End Libraries]  
    Based on T3's criteria, this task selects appropriate front-end software stacks, including CSS frameworks, UI libraries, mapping tools, and data visualization frameworks. It determines whether to use standard HTML elements or third-party solutions (e.g., Material-UI, Tailwind CSS, D3.js, Leaflet). A vector index search retrieves optimal libraries from a Neo4j-backed knowledge graph, ensuring usability, performance, and maintainability.

    \item[T6. Create Operating System Commands for Package Management Tools] After the selection of libraries in T5, our Python script retrieves the corresponding operating system (OS) commands for installing, updating, and uninstalling these libraries using the appropriate package management tools. For example, JavaScript and TypeScript dependencies can be managed using NPM and NVM, while Python libraries are handled through Pip and Conda, and system-level packages through APT (for Debian-based systems) or Yum (for RHEL-based systems). The script generates multiple package management OS commands for handling multiple dependencies in a sequence. These commands are then consolidated and exported into OS script files, such as .sh or .bash, enabling one-stop-shop execution for package management tasks under different Dev/Ops environments (Windows or Linux), including installation, version control, and conflict resolution, through the use of dedicated package management tools.
    \item[T7. Apply Software Design \& Architecture Patterns]  
    This task ensures adherence to maintainable, scalable, and modular software design principles by incorporating patterns like **Separation of Concerns (SoC), MVC, and MVVM**. It utilizes industry-standard frameworks (e.g., React, Angular) and structured prompt templates to guide LLMs in generating code with proper **componentization, event binding, and state management**.

    \item[T8. Generate Software Development Prompts]  
    Expanding on T6, this task refines structured software development prompts for LLM-driven code generation. It integrates component-based development, lazy loading, and dynamic rendering while embedding sample code from the knowledge base. The prompts provide step-by-step procedural instructions, ensuring AI-generated code follows modular design principles for reusability, maintainability, and readability.
\end{description}

Our knowledge base and code repository serve as domain experts in software engineering and GIS, facilitating the translation of plain-language annotations from wireframes into structured software development strategies. By leveraging technical terminology and software engineering best practices, we provide system-based instructions with sample code, enabling AI agents to generate robust and well-structured code in the next step.

%(a) determine the software stacks, also known as software suite that include necessary packages and libraries, required to fulfil user-defined features. 
%translate the plain-language prompts to technical language and software engineering jargon     
%Additionally, it applies reusable design patterns, such as the **Singleton** pattern for managing global states and the **Observer** pattern for handling UI event propagation, ensuring the application remains robust and extensible.   
%Once extracted, the system queries a visual contextual knowledge base that contains technical implementation instructions for each GUI component. Instead of limiting output to plain HTML and JavaScript, our approach ensures compatibility with modern web development frameworks such as React and Angular, UI design frameworks like Tailwind CSS and Bootstrap, GIS mapping libraries like Leaflet and OpenLayers, and data visualization libraries such as Highcharts and D3.js. By leveraging these structured knowledge representations, the system dynamically retrieves relevant coding patterns, component structures, and best practices associated with the specified GUI elements.

\subsubsection{Knowledge Augmented Code Generation}
\label{subsec:simulations3}
The structured prompts generated from T8 are then fed into the LLM agent to enable knowledge-augmented code generation. Given the token limit constraints of LLMs, we adopt a procedure-based, iterative approach that combines rule-based Python scripting with the customized generation capabilities of LLMs. This method ensures efficient front-end code generation using the React framework, which follows the Model-View-ViewModel (MVVM) architecture, along with established software engineering conventions and React’s standard file structure. Our KAG approach entails the following tasks from T9 to T11, which are illustrated in Figure \ref{fig:kag}. 

\begin{description}
    \item[T9. Install \& Update Packages using Operating System (OS) Scripts]  
    This task automates the installation and updating of required dependencies using OS-level scripts. It ensures that all necessary packages, including Node.js, npm, and front-end libraries (e.g., React, Material-UI, Leaflet), are properly installed and version-controlled. The scripts also handle package updates to maintain compatibility with evolving software frameworks and dependencies.

    \item[T10. Iteration-based Code Generation using LLMs]  
    Given the token limitations of LLMs, this task adopts a procedure-based, iterative approach for code generation. Rule-based Python scripts and structured prompts guide the LLMs to generate React components in a stepwise manner, ensuring compliance with best practices in componentization, event handling, and state management. The iterative process allows refinement and optimization of the generated code, minimizing redundancy and improving maintainability.

    \item[T11. Separation of Concerns (SoC) using React Convention]  
    This task enforces Separation of Concerns (SoC) by structuring the generated code according to React’s MVVM architecture. The React components, logic, styles, and API handlers are modularized into separate files, ensuring that UI elements, business logic, and data handling remain distinct. This improves scalability, maintainability, and code readability while aligning with industry standards.

    \item[T12. Script Connection \& Organization in React File Structure]  
    This task organizes and connects the generated scripts following the **React file structure convention**. The components are structured within a modular directory system (e.g., `components/`, `hooks/`, `services/`, `contexts/`). The script integration ensures that React Router, Redux (if applicable), and event-driven logic** are properly linked, allowing seamless front-end development with maintainable and reusable components.
\end{description}

\begin{figure*}[htbp]
 \centering
\includegraphics[width=\textwidth]{Figures/Figure_KAG_genreation.pdf}
 \caption{A procedure-based, knowledge-augmented code generation process that aligns with the conventions and best practices of the React framework. }
 \label{fig:kag}
\end{figure*}


After a complete React project is generated through our knowledge-augmented LLMs, two additional procedures are required before proceeding to the DevOps stage to ensure the generated code is functional, maintainable, and ready for deployment. These procedures include the following:
\begin{description}
    \item[Expert Code Review: Human-AI Collaboration for Code Refinement: ] We propose and demonstrate a Human-AI collaboration approach to refine and validate the AI-generated React code. Human experts review, debug, and revise the code to ensure correctness, performance, and adherence to industry standards. Since our method follows software engineering conventions aligned with React’s MVVM architecture, the Separation of Concerns (SoC) and code organization mirror best practices familiar to software engineers proficient in React or similar front-end frameworks. This structured design enhances the readability and interpretability of the AI-generated code, making it easier for developers to understand, modify, and integrate into production environments.
    \item[Build React Project: ] 
    Executing OS Scripts and Dependency Installation
    Once the code is validated, the React project needs to be built and configured for execution. The human user installs all required packages by running the OS scripts generated in T9 via the OS command line in either a Windows or Linux environment. This ensures all necessary dependencies, including React, Material-UI, Leaflet, and other front-end libraries, are correctly installed and up to date. After dependencies are set up, the user builds the project using NPM or NPX commands, ensuring a fully functional front-end dashboard.
\end{description}
 
For deployment, the AI-generated React project can be hosted on a server using a monolithic architecture or deployed within a Docker container as a front-end component in a microservice architecture. This ensures scalability, portability, and interoperability with other web applications, such as databases and server-side APIs. By adopting this approach, AI-generated front-end components can be seamlessly integrated into existing enterprise systems, enhancing efficiency, maintainability, and modularity.

 



 
